Sharp error bounds for imbalanced classification: how many examples in the minority class?

When dealing with imbalanced classification data, reweighting the loss function is a standard procedure allowing to equilibrate between the true positive and true negative rates within the risk measure. Despite significant theoretical work in this area, existing results do not adequately address a main challenge within the imbalanced classification framework, which is the negligible size of one class in relation to the full sample size and the need to rescale the risk function by a probability tending to zero. To address this gap, we present two novel contributions in the setting where the rare class probability approaches zero: (1) a non asymptotic fast rate probability bound for constrained balanced empirical risk minimization, and (2) a consistent upper bound for balanced nearest neighbors estimates. Our findings provide a clearer understanding of the benefits of class-weighting in realistic settings, opening new avenues for further research in this field.

==> fast_rates.tex <==
\subsection{A concentration Bound for Balanced Measures}



We now  state and prove  a concentration inequality that is key to obtain  fast convergence rates for the  excess risk in the context of balanced ERM. Prior to stating this result, we introduce notations relative to weighted classes of functions and excess risks relative to those classes.
Recall $\mathcal{G}$ is a family of real-valued score functions defined on $\mathcal{X}$. Given a loss function $\ell:\mathcal{Y}\times\mathcal{Y}\to\rset$, and  $q\in(0,1)$,  %  define the loss class
% $\mathcal{L} = \{ \ell_g, g\in \mathcal{G}\}$
%over $\mathcal{X}\times \mathcal{Y}$, where $\ell_g(x,y) = \ell(g(x), y)$. For any real number $q\in(0,1/2)$
It will be convenient to handle a  weighted loss $\tilde \ell_{q,g} =   (1-q)\ell_gI_+ + q \ell_gI_- $  where
$\ell_gI_s(x,y) = \ell(g(x),y)\un{y=s.1 }$ for $s\in\{+,-\}$, and a weighted loss class
$\mathcal{L}_q = \{ (1-q)\ell_gI_+ + q \ell_gI_- \, , g\in\mathcal{G}\} = \{ \tilde \ell_{q,g}, g \in \mathcal{G} \}$. We asssume throughout for simplicity that
for each $q$,   a  minimizer $g^*_q \in \argmin_{g\in \mathcal{G}} P\tilde \ell_{q,g}$ exists. 
Define now the excess weighted loss class
$\mathcal{F}_q = \{ \tilde \ell_{q,g} - \tilde \ell_{q, g^*_q}\}$ and notice already that by construction for all $q$, for all $f_q\in \mathcal{F}_q$, $P f_q \ge 0$.
With these notations, the AM risk writes $\mathcal{R}_{\text{bal}}(g) =  \frac{1}{2p(1-p)} P\tilde \ell_{p,g}$.  We shall obtain fast rates  under a 'Bernstein' assumption regarding the class
$\tilde{ \mathcal{F}} = \bigcup_{q\in (0,1)}\mathcal{F}_q $, namely
\begin{enumerate}[label=(B\arabic*) , wide=0.5em,  leftmargin=*]
  \item  \label{cond:bernsteinFtilde} $\exists B>0$ such that  $Pf^2 \le B Pf$, for all $f\in \tilde{ \mathcal{F}}$.
  \end{enumerate}

  Condition~\ref{cond:bernsteinFtilde}, which holds uniformly over $q\in(0,1)$,  derives immediately from commonly used  convexity and Lipschitz- properties regarding the single  loss class $\mathcal{L} = \{\ell_g,g\in\mathcal{G}\}$, as shown next. The proof is deferred to the Supplementary material
  \begin{lemma}[Sufficient conditions for the Bernstein-condition~\ref{cond:bernsteinFtilde}]\label{lemma:bernstein-cond}
    Assume that $\mathcal{G}$ is a convex subset of a normed vector
    space, and that there exists $L,\lambda>0$, such
    that for $s\in \{+1, -1\}$
    the functions $ g\mapsto P\ell_g I_s $, $s\in\{-,+\}$ %$ g\mapsto P\ell_g I_+ $, $ g\mapsto P\ell_g I_- $
    are  %$\lambda$-strongly convex. %
    respectively $p\lambda$-strongly convex and
     $(1-p)\lambda$-strongly convex.
    Assume also that for
    $g_1,g_2\in\mathcal{G}$, % $\sqrt{ P( (\ell_{g_1} - \ell_{g_2})^2I_s )} \le  L \|g_1
     % - g_2\|$, $s = +,-$. 
     $\sqrt{ P( (\ell_{g_1} - \ell_{g_2})^2I_+ )} \le \sqrt{p} L \|g_1
     - g_2\|$ and
     $\sqrt{ P( (\ell_{g_1} - \ell_{g_2})^2I_- )} \le \sqrt{1-p} L
     \|g_1 - g_2\|$.
    Then $\tilde{ \mathcal{F}}$
    satisfies~\ref{cond:bernsteinFtilde} with $B = L^2/\lambda$.
  \end{lemma}
    \begin{example}\label{example:linear}
    % \as{l'exemple d'anass (qui s'appelait Assumption 1, il faut l'appeler plutpôt exemple) fonctionne bien, comme on a discuté avec françois et j'ai vérifié. on va copier coller lancienne assumption 1 ici. }
   Assume that the domain $\mathcal{X}$ is bounded in $\rset^d$ \ie, there exists
  some $\Delta_X>0$ such as
  $\forall x \in \mathcal{X}, \left\|x\right\|\leq \Delta_X $ for some 
   norm $ \|\cdot\|$. Consider the family of classifier and
  the loss function 
  $\mathcal{G}_u=\left\{g_\beta: x\mapsto \beta^Tx \, \,  \left\|\beta\right\|\leq
    u\right\}$ and $\ell_{g_\beta}(X,Y) =\phi(\beta^T XY)$, where $\phi: \rset \mapsto \rset $ is a  twice continuously
  differentiable function which is $\mu$-strongly convex %   whose Hessian matrix $\phi^{''}$ verifies 
  % $\inf_{\abs{x}\leq u\Delta_X}\|\phi^{''}\|_{HS}(x)>\lambda$ 
  for some
  $\mu>0$. Then we have that % $\sup_{x,y \in \mathcal{X}\times \mathcal{Y}}\left\|\frac{\partial}{\partial g} \ell_g(x,y)\right\| = D <\infty$
  the domain $ I = \{ \beta^\top x y\,,, \|\beta\|\le u, x \in \Delta_x, y\in\{-1,+1\} \}$ is a subset of some bounded interval $[-M,M]$ and the derivative $\phi'$ satisfies $\sup_{t\in Y} |\phi'| =D<\infty$. 
   % , and the strong convexity assumption is also satisfied by the condition on $\phi''$.
  Direct computations show that the Lipschitz and convexity
  constraints in Lemma~\ref{lemma:bernstein-cond} are respectively
  $L = D \sigma_{\max}$, %\sqrt{1-p},
  where $\sigma_{\max}^2$ is the maximum eigenvalue of the second
  moment matrices of each class
  $V_s = \EE[XX^\top\,|\, Y= s.1], s = +, -$ ; and
  $\lambda = \mu \sigma_{\min}^2$, % p
  where $\sigma_{\min}^2$ is the minimum eigenvalue of $V_+,
  V_-$. Under the condition that each class distribution is non
  degenerate, \ie does not concentrate on any lower-dimensional
  subspace of $\rset^d$, we have $\sigma_{\min}>0$, thus
  $\lambda>0$. The assumptions of Lemma~\ref{lemma:bernstein-cond} are
  thus satisfied, so that Condition~\ref{cond:bernsteinFtilde} holds
  true with
  $$B = L^2/\lambda = \frac{D^2\sigma_{\max}^2 }{\mu\sigma_{\min}^2 }. $$
  % \as{ et là on est foutus car $B$  scale en $1/p$, ça explose. Si au contraire, dans le lemme~\ref{lemma:bernstein-cond} on modifie les constantes en $p\lambda$, $(1-p)\lambda$, et $\sqrt{p} L^$, $\sqrt{1-p} L$ alors la preuve du lemme ne fonctionne plus. Conséquence négative: on a des vitesse d'exces de risque en $1/(np^2) $ et c'est exactement ce qu'on prétend éviter. }
  % . More
  % precisely % \as{rajouter ici les calculs des constantes d'Anass}
  \end{example}

% its counterpart regarding the original  
% define a weighted class $\widetilde{\mathcal{F}}$ as
% $$\widetilde{\mathcal{F}}=\left\{\frac{1}{2}f I_{1} + \frac{1}{2}\frac{p}{1-p}f I_{-1} \mid f \in \mathcal{F}\right\},$$
% where $I_{s}(x,y)=\indic{y= s}$ for $(x,y)\in \mathcal{X}\times \mathcal{Y}$ and $s\in\{-1,1\}$. Moreover, for a given measure $P$, we denote a  balanced counterpart of $P$  as $P_{\mathrm{bal}}(f)=  \left(P_{+}(f)+P_{-}(f)\right) /2$. % At this point, we are prepared to present the primary instrument for achieving rapid convergence rates.
  
Another useful property of $\tilde{ \mathcal{F}}$ is that  it inherits % its components $\mathcal{F}_q$  inherit
the regularity property of $\mathcal{L}$, see the Supplementary material for details. 
\begin{lemma}[VC-property of $\tilde{\mathcal{F}}_q$]\label{lemma:VC-tildeF}
  If $\mathcal{L} = \{\ell_g, g\in\mathcal{G}\}$ is of VC-type with
  envelope $U$ and parameters $(v,A)$ then $\tilde{\mathcal{ F}}$ also is VC with
  envelope $2U$ and parameters  $(\tilde v = 4v+1, \tilde A = 6A)$.  %  for any $q\in(0,1)$, ${\mathcal{ F}}_q$
  % is of $VC$-type with envelope $2U$ and parameters $(v,A)$, and
  % . \as{verifier les parametres
  %   v,A} % envelope $U$ and parameters $(\tilde v,\tilde A)$ with $\tilde v = \dots$ and $\tilde A = \dots$.
  % \as{Je n'arrive pas à montrer que $\tilde{\mathcal{F}}$ est VC et je
  %   crois que ce n'est pas vrai, par exemple à cause du Théoreme 1.4
  %   dans \cite{mendelson2001size} (car c'est un log(covering), cf
  %   aussi eles résultats sur les VC-hull classes de Van der vaart) }
\end{lemma}

For $q\in(0,1)$ and $f$ a function on $\mathcal{X}\times\{-1,1\}$ let
$$P_q f = \frac{1}{2}\Big(\frac{1}{q} P fI_+ + \frac{1}{1-q} P fI_- \Big) ,$$ and let
$P_{n,q}$ denote the  empirical version
$P_{n,q} f = \frac{1}{2}(\frac{1}{q} P_n fI_+ + \frac{1}{1-q} P_n fI_- ) $.  
\begin{theorem}\label{theo:fast-rates}
  Let  $(\mathcal{ F}_q, \, q \in (0,1))$  be  a family of  classes of functions on $\mathcal{X}\times\{-1,1\}$  with common envelope $2U>0 $ % \as{modifier preuve $2U/U$ }
  such that the class $\tilde{\mathcal{F}} = \bigcup_q\mathcal{F}_q $ %\{q f  I_+ + (1-q) f I_-, q\in(0,1), f\in\mathcal{F}_q \}$
  is of VC type with parameters $(\tilde v, \tilde A)$, and that $\tilde{\mathcal{F}}$ satisfies Bernstein  condition~\ref{cond:bernsteinFtilde} for some $B\ge 2U$. 
  % and parameters $(v,A) $. Let $\tilde v,\tilde A$ be the VC-parameters of $\tilde{\mathcal{ F}}$ as given in Lemma~\ref{lemma:VC-tildeF};  Assume that there is some constant $B\geq 2 U$ such that $\tilde{\mathcal{F}}$ satisfies Condition~\ref{cond:bernsteinFtilde}, so that for every $q\in(0,1)$,  $f   \in {\mathcal{F}}_q,   P ( f^2) \leq B P f$. %let $q\in(0,1)$ be fixed. 
	Then for any $K>1$ and every $\delta >0$, with probability at least $1 - \delta $, for all $q \in (0,1)$ and $f\in\mathcal{F}_q$, % \as{on n'a pas besoin du $3\delta$ maintenant}
	\begin{align*}
P_q (f)\leq \frac{K}{K-1}P_{n,q}(f) % \left(1+\sqrt{\frac{3\log ( 1 / \delta ) }{np}}
          %\right)
         % &\\
	+ \frac{ c_1 B  K    \tilde v \log(  5\tilde A  \sqrt{ n }  / \delta  )    }{nq(1-q)} , &
	\end{align*}
	where 
$c_1>0$ is an explicit universal constant given in the proof. Also, with probability at least $1 - \delta $, $ \forall f \in \tilde{\mathcal{F}}$, 
	\begin{align*}
 P_{n} (f) % \left(1-\sqrt{\frac{2 \log ( 1 / \delta ) }{n}}\right)
          \leq \frac{K+1}{K}P(f) %	&\\
	+ \frac{ c_1 B  K    \tilde v \log(  5\tilde A  \sqrt{ n }  / \delta  )    }{nq(1-q)} .  &
	\end{align*}
  %  }
  
\end{theorem}
% \begin{theorem}\label{theo:fast-rates}
%  % \as{Modifié: l'énoncé fait intervenir $Pf, f \in \mathcal{F}_q$ où cette fois $\mathcal{F}_q$ est bien la classe des différences,et  on laisse tomber $ P_{bal} $ }
%  % {\color{red} nouveau: \\
% Suppose that $\mathcal L$  is of VC-type with envelope $U>0 $ and parameters $(v,A) $. Let $\tilde v,\tilde A$ be the VC-parameters of $\tilde{\mathcal{ F}}$ as given in Lemma~\ref{lemma:VC-tildeF};  Assume that there is some constant $B\geq 2 U$ such that $\tilde{\mathcal{F}}$ satisfies Condition~\ref{cond:bernsteinFtilde}, so that for every $q\in(0,1)$,  $f   \in {\mathcal{F}}_q,   P ( f^2) \leq B P f$. %let $q\in(0,1)$ be fixed. 
% 	For any $K>1$ and every $\delta >0$, with probability at least $1 - \delta $, for all $  f \in \tilde {\mathcal{F}} $, % \as{on n'a pas besoin du $3\delta$ maintenant}
% 	\begin{align*}
% P (f)\leq \frac{K}{K-1}P_{n}(f) % \left(1+\sqrt{\frac{3\log ( 1 / \delta ) }{np}}
%           %\right)
%          % &\\
% 	+ \frac{ c_1 B  K    \tilde v \log(  5\tilde A  \sqrt{ n }  / \delta  )    }{n} , &
% 	\end{align*}
% 	where 
% $c_1>0$ is an explicit universal constant given in the proof. Also, with probability at least $1 - \delta $, $ \forall f \in \tilde{\mathcal{F}}$, 
% 	\begin{align*}
%  P_{n} (f) % \left(1-\sqrt{\frac{2 \log ( 1 / \delta ) }{n}}\right)
%           \leq \frac{K+1}{K}P(f) %	&\\
% 	+ \frac{ c_1 B  K    \tilde v \log(  5\tilde A  \sqrt{ n }  / \delta  )    }{n} .  &
% 	\end{align*}
%   %  }
%     \as{On pourrait faire un énoncé plus général avec une classe $\mathcal{F}$ quelconque vérifiant bernstein, pour l'instant on laisse et on verra plus tard quand le reste ira bien. }
% \end{theorem}


\begin{proof}[Sketch of proof]

  The main tool for the proof is % proof of Theorem \ref{theo:fast-rates} relies  on applying
  Theorem 3.3  in \cite{Bartlett2005} recalled for completeness in the supplementary material (Theorem \ref{theo:fast-rates-ingredient}).
  The argument from the cited reference relies on a fixed point technique relative to a sub-root function upper bounding some local Rademacher complexity. %  with localized variance $P (f'^2) \leq r$.  
  % We establish an explicit upper-bound on the local Rademacher complexity of $\mathcal{F}'$ (Lemma~\ref{lemma:sub-root-UB2}), which is a subroot function $\psi$  of the localizing parameter $r$. 
  We establish that the  fixed point of the subroot function is  of order $O(\log(n)/n)$.   %  we establish that the fixed point $r^\star$ involved in the argument  satisfies an inequality of the following simplified form
  % $$r^\star \leq   \sqrt { r ^*  \frac{\log(n)}{n}  }  +    \frac{\log(n)}{n}  $ 
% {\color{blue} supprimer ce sketch pas vraiment informatif: and this yields a result of the following form, with high probability, for all $\tilde f \in \widetilde{\mathcal{F}}$,
% 	 $$ P(\tilde f)\leq \frac{K}{K-1}P_{n}(\tilde f)+  \frac{\log(n)}{n} .$$
%          It remains to notice that in our context of imbalanced classification, for $$\tilde f = \frac{1}{2}f I_{1} + \frac{1}{2}\frac{p}{1-p}f I_{-1},$$ one has $P(\tilde f)=pP_{\mathrm{bal}}(f)$. The result follows by an application of a Chernoff bound (Theorem \ref{th_chernoff}) % (Therefore, if we divide by $p$ the latter inequality and use  we get the desired result.
%        }
 %{\color{red}  nouveau: %In addition, an explicit subroot function is shown to upper bound a local Rademacher process of the class, with an explicit fixed point.
 Plugging the expression of the fixed point $r^\star$ in the upper bounds from~\cite{Bartlett2005} concludes the argument. %}
The full proof can be found in the supplement, in Section \ref{sec:fast-rates-proof}.
\end{proof}
% %\as{todo expliquer mieux (corollaire? ) que:
% Theorem~\ref{theo:fast-rates} has important consequences in terms of
% weighted risks.

% For
% $f = \tilde \ell_{q,g} - \tilde \ell_{q,g_q^*} \in
% \mathcal{F}_q\subset \tilde{\mathcal{F}}$, the quantity $Pf$
% is an excess weighted risk up to a scaling factor. % for the score functions $g$. Namely,
% Indeed
% % With
% % these notations, 
% the bound in Theorem~\ref{theo:fast-rates} when
% rescaled by $q(1-q)$ immediately yields the following fast rate result
% relative to $(nq)$ (as $q\ll 1$): with probability $1-\delta$,
%   \begin{equation}
%     \label{eq:boundDeviationExcessRq}
%   \begin{gathered}
% \forall g\in\mathcal{G}, \forall q\in(0,1), \mathcal{R}_{q}(g) - \mathcal{R}_q(g_q^*) \le \\
% \frac{K}{K-1} (\mathcal{R}_{n,q}(g) - \mathcal{R}_{n,q}(g_q^*) ) % \left(1+\sqrt{\frac{3\log ( 1 / \delta ) }{np}}
%           %\right)
%          % &\\
% 	+ \frac{ c_1 B  K    \tilde v \log(  5\tilde A  \sqrt{ n }  / \delta  )    }{2nq(1-q)} .  
%   \end{gathered}  
% \end{equation}

\begin{discussion*}
	 Similar proof techniques can be found in the standard classification literature, for example Corollary 3.7 in \cite{Bartlett2005}. Nevertheless, this particular work primarily concentrates on loss functions with binary values, namely $\left\{0,1\right\}$. The proof is based upon the fact that these functions are positive, and it employs the initial definition of the \VC dimension \citep{vapnik71}. In contrast, other existing works (e.g. Theorem 2.12 in \cite{bartlett2006empirical} or Example 7.2 in \cite{Gine2006}) demonstrate accelerated convergence rates for the \textit{typical} empirical risk minimizers, which do not extend to their balanced counterparts. The present result is more general, as it is uniformly applicable to a broader range of bounded functions and encompasses a more extensive definition of the \VC class. This notable extension facilitates the establishment of fast convergence rates for the excess risk of  (\ML) algorithms employed in imbalanced classification scenarios, such as cost-sensitive logistic regression and balanced boosting \citep{Menon2013,koyejo2014consistent,Tanha2020,xu2020class}.  In the remainder of this  section we provide examples of algorithms that verify the assumptions  of Theorem \ref{theo:fast-rates}.
\end{discussion*}



 %For simplicity we limit ourselves to the simplified setting of Example~\ref{example:linear}. % The following assumption, known as the Bernstein condition, is a prevalent concept within the fast rates literature \citep{bartlett2006empirical,klochkov2021stability}.
% \begin{definition}\label{assum:bernstein-condition} \as{supprimer car on utilise condition~\ref{cond:bernsteinFtilde} qui veut dire pareil mais en plus clair}
% 	We say that the triplet $(\mathcal{G},P,\ell)$
% 	satisfies the  Bernstein condition if for some $B > 0$ it holds that, $\forall g\in\mathcal{G}$,
% 	\begin{align*}
% 		 \EE\Big[\left(\ell_g(X,Y)-\ell_{g^\star}(X,Y)\right)^2&\Big]\leq  B \left(\risk(g)-\risk(g^\star)\right),
% 	\end{align*}
% 	where $g^\star=\argmin_{g\in\mathcal{G}}\risk[g]=\argmin_{g\in\mathcal{G}}\EE\left[\ell_g(X,Y)\right]$.
% \end{definition}
% Set $$\tilde \ell_g =\ell_g I_{1} +\frac{p}{1-p}\ell_g I_{-1}, $$ and notice that $\risk_{\mathrm{bal}}\left(g\right)=\EE\left[\tilde\ell_g(X,Y)\right]/p$,  so that
% $$g^\star_{\mathrm{bal}}=\argmin_{g\in\mathcal{G}}P (\tilde\ell_g)=\argmin_{g\in\mathcal{G}}\risk_{\mathrm{bal}}\left(g\right).$$
% %The same remark holds also for $\hat g_{\mathrm{bal}}$, that is ,
% %$$ \hat g_{\mathrm{bal}}=\argmin_{g\in\mathcal{G}}P_n\left(\tilde\ell(g,O)\right)=\argmin_{g\in\mathcal{G}}\risk_{n,\mathrm{bal}}\left(g\right).$$
% In the sequel we shall  suppose that the latter condition holds for $(\mathcal{G},P,\tilde \ell)$  in order to apply Theorem~\ref{theo:fast-rates} and obtain fast convergence rates for the excess risk.
%
% \as{ (à re organiser car $\mathcal{R}_q$ est introduit au-dessus)}
As an application of Theorem \ref{theo:fast-rates}, we derive fast rates for the excess risk of empirical risk minimizers.
For this purpose
Consider 
   for $q\in(0,1)$  the weighted  risk with weighting parameter $q$, 
 % For $n_+\le n_- \le n$ with $n_+ + n_- = n$ consider  
    $$
 \mathcal{R}_{q}(g)  = \frac{1}{2}(\frac{1}{q }P\ell_gI_+ + \frac{1 }{(1-q)}P\ell_gI_{-1}), 
$$
% Namely consider the weighted risk using a scaling factor $q$,
% $\mathcal{R}_q(g) = \frac{1}{2}( \frac{1}{q}P \ell_gI_+ +
% \frac{1}{(1-q)} P\ell_g I_- )$,
and let $\mathcal{R}_{n,q}$ denote its
empirical counterpart, \ie
$\mathcal{R}_{n,q}(g) = \frac{1}{2}( \frac{1}{q}P_n \ell_gI_+ +
\frac{1}{(1-q)} P_n\ell_g I_- )$.  
% To wit, $q$ will be chosen as $\hat p$ in our  application to Empirical Risk Minimization (Corollary~\ref{coro:fast-rates-excessrisk}.
Notice
already that $\mathcal{R}_p  = \mathcal{R}_{\text{bal}} $ and that
$\mathcal{R}_{n, \hat p} = \mathcal{R}_{n, \text{bal}}$. 
% Finally notice that
% $ \mathcal{R}_{p} =  \mathcal{R}_{\text{bal}}$. 
% we consider a modified version of the balanced risk $\mathcal{R}_{\text{bal}} = \mathcal{R}_p$,  % (see the defnition of $\mathcal{R}_p$ above Inequality~(\ref{eq:boundDeviationExcessRq}), 
% where $p$  is replaced with $\hat p$. In other words o
Our result (Corollary~\ref{coro:fast-rates-excessrisk} below) is  stated in terms  of excess of $\mathcal{R}_{\hat p}$ risk.  %, the number of observed positive examples. % Also our statement takes the form of a tail bound on the error, conditionally on $N_+=n_+$,  with $N_+ = \sum_{i=1}^n\un{Y_i=1}$, or equivalently, conditionally on $\hat p = N_+/n$.
    % Notice that $ \mathcal{R}_{q}(g) =  P(\tilde \ell_{q, g} )/ \big(2q (1-q)\big)$. Thus the minimizers of $\mathcal{R}_{q} $ and those of $P(\tilde{ \ell}_{q, \cdot} )$ coincide.
    % Recall that  $g^*_{q}$ denotes  a minimizer of $P(\tilde \ell_{q,  \cdot } )$, or  equivalently, of $\mathcal{R}_q$. % according to the notations introduced at  the beginning of this section. 

\begin{corollary}\label{coro:fast-rates-excessrisk}
 %  \as{ %Tant qu'on ne peut pas l'énoncé est (je crois)  faux (même le nouveau)
 %    ça simplifierait  vraiment d'avoir $\tilde{\mathcal{F}}$ VC pour intervertir  le $\forall q $ avec le 'with proba $ 1-\delta$ dans le théoreme précédent. Mais  je pense que c'est faux. Heureusement on peut s'en sortir en faisant une borne de l'union sur les $N_+$ 'probables', c'est à dire dans
 %    l'intervalle $np +/- \sqrt{ 3 np \log(1/\delta) } $ par le Théoreme~\ref{th_chernoff}. Ainsi on doit choisir $\delta \le \approx 1/\sqrt{np} \approx 1/\sqrt{n_+}$ et par une borne de l'union on aura avec proba $1-\delta$ que $N_+$ est dans cet intervalle raisonnable.
 %    Donc je crois assez fort à l'énoncé ci-dessous
 %  }~\\
 % %     modifier. Ecrire à la place quelque chose conditionellement à n+, n-: par exemple : \\   
 % %     Then a minimizer of $\mathcal{R}_{n_+, n_-}$ is $g^*_q$ with $q = n_+ / n\le 1/2$.
 % {\red
  Assume that  $\mathcal{L}=\{\ell_g\, :\, g\in \mathcal G\}$ is VC-type with envelope $U>0$ and parameters $(v,A)$ and assume that $\tilde{\mathcal{F}}$ defined at the beginning of this section  satisfies the Bernstein condition~\ref{cond:bernsteinFtilde} for some $B\geq 2 U $.
 Let $\hat g_{\text{bal}}$ be  a minimizer of the empirical balanced risk $\mathcal{R}_{n, \text{bal}}$ considered in Section~\ref{sec:standard}.  % (eux ne changent pas ). Then  
  Then for $\delta>0$,  %\le \approx 1/\sqrt{np}$ \as{Préciser !} % Conditionnally to $N_+ = n_+, N_- = n_-$,  with conditional
  with probability $1-  \delta$,  %\as{preciser, cf preuve},
  \begin{align*}
& \mathcal{R}_{\hat p}(\hat g_{\text{bal}}) - \mathcal{R}_{\hat p}(g_{\hat p}^*) \le 
%\frac{ (\mathcal{R}_{n,\hat p}(g) - \mathcal{R}_{n,\hat p}(g_{\hat p}^*) ) % \left(1+\sqrt{\frac{3\log ( 1 / \delta ) }{np}}
          %\right)
          % &\\
 \frac{ c_1 B      \tilde v \log(  5\tilde A  \sqrt{ n }  / \delta  )    }{n \hat p(1-\hat p)},     \end{align*}
%}
 %    $$
 % \mathcal{R}_{\hat p}( \hat g_{\text{bal}}) \le \mathcal{R}_{\hat p }(g^*_{\hat p}) + O( \log(\sqrt{n}/\delta )/(np))
 % $$
 % \as{todo: expliciter la borne}}
 
% {\color{blue} Ancien: \\
% 	Suppose that $\mathcal{F}=\{\ell_g\, :\, g\in \mathcal G\}$ is VC-type with envelope $U>0$ and parameters $(v,A)$ and assume that $(\mathcal{F},P,\tilde \ell) $ satisfies the Bernstein condition for some $B\geq U $. Then, for any $\delta>0$,
% 	we have with probability $1- 3 \delta $,
% 	\begin{align*}
% 	\risk_{\mathrm{bal}}\left(\hat g_{\mathrm{bal}} \right) & \leq  \risk_{\mathrm{bal}}( g^\star_{\mathrm{bal}} ) 	+  \frac{ 2 c_1 B     v \log(  5A  \sqrt{ n }  / \delta  )    }{np} ,
% 	\end{align*}
where $(\tilde v = 4v+1, \tilde A = 6A)$, and where the constant $c_1$%, %\tilde v, \tilde A$ are
is the same as in Theorem~\ref{theo:fast-rates}.
\end{corollary}
\begin{proof}
  % Because %Inequality~(\ref{eq:boundDeviationExcessRq})
  We apply Theorem~\ref{theo:fast-rates} to the class
  $\mathcal{F} =  \mathcal{L} = \{\ell_g, g\in\mathcal{G}\}$ % \{\ell_{g_1}-\ell_{g_2}, g_1,g_2\in\mathcal{F}\}$, which has  envelope $2U$ if $\mathcal{L}$ has envelope $U$.    % of excess risks
  $\tilde {\mathcal{F}} = \{ \tilde \ell_{q,g} - \tilde \ell_{q,g^*_q}, g\in\mathcal{G}, q\in(0,1) \}$. Because the  result of Theorem~\ref{theo:fast-rates} 
  holds uniformly over $q\in(0,1)$, $g\in\mathcal{G}$,  one may choose $q=\hat p$ and $\hat g = \hat g_{\hat p} = \hat g_{\text{bal}}$. Then the first term on the right-hand side of~(\ref{eq:boundDeviationExcessRq}) is nonpositive, and the result follows upon choosing $K=2$.
\end{proof}
\begin{remark}[Weighting with $\hat p$ of $p$]
   % In spirit, considering $\mathcal{R}_{\hat p}$ instead of $\mathcal{R}_p$  is close to assuming that $p$ known, or that $n_+,n_-$ the numbers of positive and negative examples are fixed.  In this respect our setting for fast rates comes closer to \cite{rigollet2011neyman} compared with Section~\ref{sec:standard}, the main difference here is that our rates are fast. 
How to obtain a similar fast rate regarding $\mathcal{R}_{p} $ it self, not $\mathcal{R}_{\hat p}$, is left as an open question. The main bottleneck seems to be that replacing $\hat p$ with $p$ induces additional slow rate terms of order $O(1/\sqrt{np})$. 
  \end{remark}

%\begin{proof}
%	The proof follows in a straightforward way from Theorem \ref{theo:fast-rates}. Since Assumption \ref{assum:bernstein-condition} holds, we can apply Theorem \ref{theo:fast-rates} to the class of functions  $\mathcal{F}_1=\{\ell_g-\ell_{g^\star_\mathrm{bal}}\, :\, g\in \mathcal G\}$ and obtain, with probability $1-3\delta$,
%	\begin{align*}
%		\forall g \in \mathcal{G} \quad P_{\mathrm{bal}} (\ell_g-\ell_{g^\star_\mathrm{bal}})\leq \frac{K}{K-1}P_{n,\mathrm{bal}} (\ell_g-\ell_{g_\mathrm{bal}^\star})&\Bigg(1+\sqrt{\frac{3\log(1/\delta)}{np}}\Bigg)\\&+\frac{D K}{B} \frac{\log(An)^2}{np}+\frac{\log(1/\delta)\left(c_2+c_1 B K\right)}{np}.
%	\end{align*}
%	In particular for $\hat g_\mathrm{bal}=\argmin_{g\in\mathcal{G}} \risk_{n,\mathrm{bal}}(g)=\argmin_{g\in\mathcal{G}}P_{n,\mathrm{bal}}(g)$, we have 
%	\begin{align*}
%		P_{n,\mathrm{bal}}\left(\hat g_{\mathrm{bal}}-g^\star_\mathrm{bal}\right)= 	P_{n,\mathrm{bal}}(\hat g_{\mathrm{bal}})-P_{n,\mathrm{bal}}(g^\star_\mathrm{bal})\leq 0
%	\end{align*}
% and the result follows by reminding that $P_{\mathrm{bal}} (\ell_{\hat g_{\mathrm{bal}}}-\ell_{g^\star_\mathrm{bal}})=\risk_{\mathrm{bal}}(\hat g_{\mathrm{bal}})-\risk_{\mathrm{bal}}(g^\star_\mathrm{bal})$ and by taking $K=1$.
%\end{proof}


%\begin{remark}
%	By the remarks figuring in page 5 from \cite{klochkov2021stability} we know that, if $\ell^\prime$ is $L$ Lipschitz and  $\lambda$ strongly convex with respect to it's first argument. Then $(\mathcal{F},P,\ell^\prime) $ verifies assumption \ref{assum:bernstein-condition} with $B=2L^2/\lambda$.
%\end{remark}
%Before stating our next result, we remind the definition of $\lambda$-strongly convex function (ref)
%\begin{definition}
%	A function $f: \mathcal{X}\mapsto \rset$ is $\lambda$ strongly convex is said to be $\lambda$-strongly convex for some $\lambda>0$ if,
%	$$\forall x,y\in \mathcal{X}\,, f(y) \geq f(x)+\nabla f(x)(y-x)+\frac{\lambda}{2}\|y-x\|^2,$$
%	where $\nabla f(x)$ denotes a sub-gradient of $f$ at $x$.
%	
%\end{definition}

% In the following lemma, we provide a sufficient condition for the Bernstein assumption (Definition~\ref{assum:bernstein-condition}). 	The proof and the definition of strongly convex function is given in the supplement \as{now it's true, see proof of lemma .... } %\new{not true}.



% \begin{lemma}\label{lemma:bernstein-cond}
%   Suppose that the family $\mathcal{G}$ is a normed space. %\new{Is there really a $\mathbb E $ in the next?}
%   If $g\mapsto \EE\left[\ell_g(X,Y)\right]$ is $L$-Lipschitz and  $\lambda$-strongly convex, then $(\mathcal{F},P,\tilde \ell) $ verifies the Bernstein assumption (Definition~\ref{assum:bernstein-condition}) with $B=2L^2/\lambda$.
% \end{lemma}

We conclude this section by an illustration of the significance of our results, through the concrete setting of Example~\ref{example:linear}. 
 % a  constrained empirical risk minimization problem over a certain class of classifiers.
%  We show that  fast rates of convergence are achieved  provided that the covariate space $\mathcal{X}\subset  \mathbb {R}^d$ is bounded and the loss is twice differentiable with a second derivative lower bounded away from $0$. More precisely, we make the following assumption.
% \begin{assumption}\label{assum:strong-convexity}
%   The space $\mathcal{X}$ is bounded in $\rset^d$ \ie, there exists
%   some $\Delta_X>0$ such as
%   $\forall x \in \mathcal{X}, \left\|x\right\|\leq \Delta_X $ for a
%   given norm $ \|\cdot\|$. Furthermore, the family of classifier and
%   the loss function are chosen as 
%   $\mathcal{G}_u=\left\{g(x)=\beta^Tx\mid \left\|\beta\right\|\leq
%     u\right\}$ and $\ell_g(X,Y) =\phi(\beta^T XY)$, where $\phi: \rset \mapsto \rset $ is a  twice
%   differentiable function  verifying
%   $\inf_{\abs{x}\leq u\Delta_X}\phi^{''}(x)>\lambda$ for some
%   $\lambda>0$.
% \end{assumption}
% An immediate implication of the aforementioned assumption is that, identifying $g$ with $\beta$, we have  $\sup_{x,y}\left\|\frac{\partial}{\partial g} \ell_g(x,y)\right\|<\infty$ which ensures that the risk  is Liptchitz. In addition this assumption guarantees that the risk  is $\lambda$-strongly convex with respect to $g$.
The following corollary is a direct consequence of Corollary \ref{coro:fast-rates-excessrisk} and guarantees fast rates of convergence for constrained \ERM, specifically for algorithms of the form  $\hat g_{u,bal}(x)=\hat \beta_u^{T} x$ with
\begin{align*}
	\hat \beta_u=\argmin_{\left\|\beta\right\| \leq u} \frac{1}{n}\sum_{i=1}^{n}\phi(\beta^\top X_iY_i)&\Bigg(\frac{\mathds{1}\{Y=1\}}{{\hat p}}\nonumber\\
	&\hspace{5mm}+\frac{\un{Y=-1}}{1-{\hat p}}\Bigg).
\end{align*}
\begin{corollary}\label{coro:fast-rates-contrained} 
% \new{to adapt} \as{oui remettre les calculs de constante B de la condition~\ref{cond:bernsteinFtilde}}
% Suppose that Assumption \ref{assum:strong-convexity} holds for some $\lambda>0$.
  \as{à reecrire }
In the setting of Example~\ref{example:linear}  the excess risk of $\hat g_u$  verifies, for any $\delta>0$,
 with probability $1-4\delta$, \as{modifier le résultat}
 \begin{align*}
 \risk_{\mathrm{bal}}\left(\hat g_{\mathrm{bal}} \right)\leq \risk_{\mathrm{bal}}( g^\star_{\mathrm{bal}}&)+ \frac{D\lambda}{L'^2} \frac{\log(An)^2}{np}\\
 &+\frac{\log(1/\delta)\left(c_2+2c_1(L'^2/\lambda) \right)}{np},
 \end{align*}
	where $L'=\sup_{\abs{x}\leq u\Delta_X}\phi'(x)$.
\end{corollary}

\begin{discussion*}
In the context of constrained logistic regression, where $\phi(x) = \log(1 + e^{-x})$, the latter corollary yields fast convergence rates with constants and $L' = 1$, along with $\lambda = e^{-u}$. Corollary~\ref{coro:fast-rates-contrained} further establishes accelerated convergence rates for constrained empirical \emph{balanced} risk minimization with respect to losses such as mean squared error, squared hinge, and exponential loss, among others. This outcome aligns with expectations, as constrained empirical risk minimization is equivalent to penalization \citep{lee2006efficient,homrighausen2017risk}. Numerous studies have demonstrated the effectiveness of penalization in achieving rapid convergence rates \citep{Koren15,vanerven15a}. This aspect is particularly significant in the present context, as the standard convergence rate for imbalanced classification is $1/\sqrt{np}$, and accelerating the convergence rate leads to a more pronounced impact.
\end{discussion*}


%
%\begin{figure}[!h]
%	\centering
%	\begin{subfigure}{0.4\textwidth}
%		\includegraphics[width=\textwidth]{Excess_risk_1.pdf}
%		\caption{${\hat p}=1/n^{1/3}.$}
%		\label{fig:first}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}{0.4\textwidth}
%		\includegraphics[width=\textwidth]{Excess_risk_2.pdf}
%		\caption{${\hat p}=1/n^{1/2}.$}
%		\label{fig:second}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}{0.4\textwidth}
%		\includegraphics[width=\textwidth]{Excess_risk_3.pdf}
%		\caption{$p_n=1/n^{2/3}.$}
%		\label{fig:third}
%	\end{subfigure}
%	
%	\caption{Excess risk (blue) of logistic regression  for different sample size $n$ and the curve $1/np$ (orange). The blue area corresponds to the $0.9$-confidence interval.}\label{fig:excessrisk}.
%	\label{fig:figures}
%\end{figure}






%
%\begin{proof}
%
%\textbf{OLD STUFF}
%Since the previous class is parametric, the entropy condition to apply Theorem 2 holds. 
%
%	We further suppose that $\hat \beta \to \beta_0$ in probability (a result that shall be obtained). Under the stipulated assumptions one has
%	$$ P_n \left(\nabla \ell_{\hat \beta}  \mid A\right) + P_n\left(\nabla \ell_{\hat \beta}  \mid B\right) =  0$$
%	and 
%	$$ P\left(\nabla \ell_{ \beta _0 } -\nabla \ell_{ \beta_0}  \mid  A\right) + P\left(\nabla \ell_{ \beta _0 } -\nabla \ell_{ \beta_0} \mid B \right) =  0$$
%	We have 
%	$$ P_n \left(\nabla \ell_{\hat \beta} -\nabla \ell_{ \beta_0}   \mid A\right) + P_n \left(\nabla \ell_{\hat \beta}-\nabla \ell_{ \beta_0}  \mid B\right) =  -P_n \left(\nabla \ell_{ \beta_0}  \mid A\right) - P_n \left(\nabla \ell_{\beta_0} \mid B\right)$$
%	And hence 
%	$$ P\left(\nabla \ell_{\hat \beta} -\nabla \ell_{ \beta_0}   \mid A\right) + P\left(\nabla \ell_{\hat \beta}-\nabla \ell_{ \beta_0}   \mid B\right) =  -P_n \left(\nabla \ell_{ \beta_0}  \mid A\right) - P_n \left(\nabla \ell_{\beta_0}  \mid B\right) + \Delta_n$$
%	with 
%	$$\Delta_n = \left(P_n - P\right) \left(\nabla \ell_{\hat \beta} -\nabla \ell_{ \beta_0} \mid A \right) + \left(P_n - P\right) \left(\nabla \ell_{\hat \beta} -\nabla \ell_{ \beta_0} \mid B \right).$$
%	Invoking the weak convergence property in Theorem 2 we have that (to be done rigourously) $\Delta_n = o_p\left( 1/\sqrt{nP(A)} + 1 / \sqrt {nP(B)}\right)$. 
%	
%	
%	It follows using a Taylor development that
%	$$ \left(P \left(\nabla^2 \ell_{\tilde \beta}  \mid A\right) + P\left(\nabla^2 \ell_{\tilde \beta}  \mid B\right)\right) \left(\hat \beta - \beta_0\right) = -P_n \left(\nabla \ell_{ \beta_0}  \mid A\right) - P_n \left(\nabla \ell_{\beta_0}  \mid B\right) +\Delta_n $$
%	This implies that
%	$$ \left(H + o_P(1)\right) \left(\hat \beta - \beta_0\right) = -P_n \left(\nabla \ell_{ \beta_0}  \mid A\right) - P_n \left(\nabla \ell_{\beta_0}  \mid B\right) $$
%	Moreover using $\sqrt{n P(B) } \nabla \ell_{ \beta_0}  | A) = O_{p} (\sqrt{P(B) / P(A)}) = o_p(1)$, it follows that
%	$$ (H + o_P(1)) \sqrt{n P(B) } (\hat \beta - \beta_0) = - \sqrt{n P(B) } P_n (\nabla \ell_{\beta_0}  | B)  + o_P(1)$$
%	from which we can deduce the result.
%\end{proof}



 	
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main-imbalanced"
%%% End:

